VLASH: Real-Time VLAs via Future-State-Aware Asynchronous Inference

Vision-Language-Action models (VLAs) are becoming increasingly capable across diverse robotic tasks. However, these models are typically deployed under synchronous inference, where the robot waits for model inference to complete before acting, and cannot perceive or respond to environmental changes during action execution. This not only introduces noticeable action stalls, but also significantly increases reaction latency, fundamentally limiting the applicability of VLAs to dynamic, real-time tasks. Asynchronous inference offers a promising solution to achieve continuous and low-latency control by enabling robots to execute actions and perform inference simultaneously. However, because the robot and environment continue to evolve during inference, a temporal misalignment arises between the prediction and execution intervals. This leads to significant action instability, while existing asynchronous methods either degrade accuracy or introduce runtime overhead to mitigate it. We propose VLASH, a simple yet effective method for asynchronous VLA inference that delivers smooth, accurate, and fast reaction control without architectural changes or additional runtime overhead. VLASH leverages the future execution-time state by rolling the robot state forward with the previous action chunk, thereby bridging the gap between prediction and execution. Experiments show that VLASH reduces reaction latency by up to 11.8x compared to synchronous inference and consistently outperforms all asynchronous baselines in accuracy. With action quantization, it further achieves 1.5-2.0x task completion speedup with minimal accuracy loss. Moreover, it empowers state-of-the-art VLAs such as $\pi_{0.5}$ to handle fast-reaction, high-precision tasks including playing ping-pong and playing whack-a-mole, where traditional synchronous inference fails. Code is available at https://github.com/mit-han-lab/vlash

==> sec/teaser.tex <==
\makeatletter
\let\@oldmaketitle\@maketitle
\renewcommand{\@maketitle}{%
  \@oldmaketitle
  \begin{center}
    \captionsetup{type=figure}
    \setcounter{figure}{0}
    \includegraphics[width=0.161\textwidth]{figs/teaser/frame_000150.png}
    \includegraphics[width=0.161\textwidth]{figs/teaser/frame_000155.png}
    \includegraphics[width=0.161\textwidth]{figs/teaser/frame_000160.png}
    \includegraphics[width=0.161\textwidth]{figs/teaser/frame_000163.png}
    \includegraphics[width=0.161\textwidth]{figs/teaser/frame_000165.png}
    \includegraphics[width=0.161\textwidth]{figs/teaser/frame_000170.png}
    \captionof{figure}{\textbf{\method enables a VLA to play ping-pong rallies with humans.} Snapshots showing $\pi_{0.5}$~\cite{intelligence2025pi_} with \method tracking and striking a fast-moving ping-pong ball during a rally. The robot initiates its reaction by the third frame, demonstrating low-latency response. The task requires fast reaction and smooth continuous motion, which are enabled by asynchronous inference with \textit{future-state-awareness}. Under synchronous inference, the robot fails to achieve this dynamic interaction.}
    \vspace{-4mm}
    \label{fig:teaser}
  \end{center}
}
\makeatother

